Data-driven dynamic treatment planning for chronic diseases

In order to deliver effective care, health management must consider the distinctive trajectories of chronic diseases. These diseases recurrently undergo acute, unstable, and stable phases, each of which requires a different treatment regimen. However, the correct identification of trajectory phases, and thus treatment regimens, is challenging. In this paper, we propose a data-driven, dynamic approach for identifying trajectory phases of chronic diseases and thus suggesting treatment regimens. Specifically, we develop a novel variable-duration copula hidden Markov model (VDC-HMMX). In our VDC-HMMX, the trajectory is modeled as a series of latent states with acute, stable, and unstable phases, which are eventually recovered. We demonstrate the effectiveness of our VDC-HMMX model on the basis of a longitudinal study with 928 patients suffering from low back pain. A myopic classifier identifies correct treatment regimens with a balanced accuracy of slightly above 70%. In comparison, our VDC-HMMX model is correct with a balanced accuracy of 83.65%. This thus highlights the value of longitudinal monitoring for chronic disease management.

==> correlations_main.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Mon Jan 15 17:32:32 2018
 0 & \cellcolor{black}\color{white}77.71 & 4.46 & 7.09 & 5.41 & 2.79 & 1.53 & 0.63 & 0.27 & 0.10 & 0.02 & 0.01 \\ 
  1 & 0.51 & 8.98 & \cellcolor{black!40}25.38 & \cellcolor{black!40}25.53 & \cellcolor{lightgray!40}16.14 & \cellcolor{lightgray!40}11.32 & 5.69 & 3.91 & 1.98 & 0.30 & 0.25 \\ 
  2 & 0.12 & 2.85 & \cellcolor{lightgray!40}17.47 & \cellcolor{lightgray!40}22.71 & \cellcolor{lightgray!40}19.92 & \cellcolor{lightgray!40}16.31 & \cellcolor{lightgray!40}10.19 & 5.42 & 4.25 & 0.64 & 0.12 \\ 
  3 & 0.09 & 1.48 & 8.68 & \cellcolor{lightgray!40}20.14 & \cellcolor{lightgray!40}20.23 & \cellcolor{lightgray!40}22.14 & \cellcolor{lightgray!40}11.63 & 8.68 & 5.21 & 1.22 & 0.52 \\ 
  4 & 0.13 & 0.80 & 5.59 & 9.32 & \cellcolor{lightgray!40}19.97 & \cellcolor{black!40}26.36 & \cellcolor{lightgray!40}16.91 & \cellcolor{lightgray!40}11.19 & 7.59 & 1.86 & 0.27 \\ 
  5 & 0.29 & 1.17 & 5.98 & 7.43 & \cellcolor{lightgray!40}12.10 & \cellcolor{lightgray!40}23.62 & \cellcolor{lightgray!40}16.18 & \cellcolor{lightgray!40}16.76 & \cellcolor{lightgray!40}12.83 & 2.62 & 1.02 \\ 
  6 & 0.00 & 0.00 & 5.30 & 3.03 & 6.44 & \cellcolor{lightgray!40}15.91 & \cellcolor{lightgray!40}25.00 & \cellcolor{lightgray!40}17.05 & \cellcolor{lightgray!40}19.70 & 3.79 & 3.79 \\ 
  7 & 0.14 & 5.73 & \cellcolor{lightgray!40}11.09 & \cellcolor{lightgray!40}10.57 & \cellcolor{lightgray!40}11.88 & \cellcolor{lightgray!40}16.06 & \cellcolor{lightgray!40}13.34 & \cellcolor{lightgray!40}13.95 & \cellcolor{lightgray!40}11.51 & 2.58 & 3.15 \\ 
  

==> mvt_emission.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Oct 07 13:26:16 2019
 0 & \cellcolor{black}\color{white} 99.9 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \cellcolor{black!40} 6.3 & 0.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.2 & 0.2 & 0.1 & 0.1 & 0.1 & 0.0 & 0.0 & 0.1 \\ 
  1 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \cellcolor{black!40} 15.8 & \cellcolor{lightgray!40} 2.1 & 0.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 & 0.7 & 0.7 & 0.6 & 0.4 & 0.3 & 0.1 & 0.8 \\ 
  2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \cellcolor{black!40} 19.3 & \cellcolor{lightgray!40}4.6 & 0.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 & \cellcolor{lightgray!40} 1.3 &\cellcolor{lightgray!40} 1.7 &\cellcolor{lightgray!40} 1.6 & \cellcolor{lightgray!40} 1.2 & 0.8 & 0.4 & \cellcolor{lightgray!40} 2.3 \\ 
  3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \cellcolor{black!40}15.4 & \cellcolor{black!40} 5.8 & 0.8 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 &\cellcolor{lightgray!40} 1.4 &\cellcolor{lightgray!40} 2.5 &\cellcolor{lightgray!40} 2.6 &\cellcolor{lightgray!40} 2.1 &\cellcolor{lightgray!40} 1.4 & 0.8 &\cellcolor{lightgray!40} 4.3 \\ 
  4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \cellcolor{black!40} 9.2 &\cellcolor{lightgray!40} 4.8 & 0.8 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 &\cellcolor{lightgray!40} 1.4 &\cellcolor{lightgray!40} 2.6 &\cellcolor{lightgray!40} 3.0 &\cellcolor{lightgray!40} 2.6 &\cellcolor{lightgray!40} 1.7 &\cellcolor{lightgray!40} 1.0 & \cellcolor{black!40} 5.8 \\ 
  5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 &\cellcolor{lightgray!40} 4.4 &\cellcolor{lightgray!40} 2.9 & 0.6 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 &\cellcolor{lightgray!40} 1.1 &\cellcolor{lightgray!40} 2.3 &\cellcolor{lightgray!40} 2.8 &\cellcolor{lightgray!40} 2.5 &\cellcolor{lightgray!40} 1.7 &\cellcolor{lightgray!40} 1.0 & \cellcolor{black!40} 6.1 \\ 
  6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 &\cellcolor{lightgray!40} 1.8 &\cellcolor{lightgray!40} 1.4 & 0.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.2 & 0.8 &\cellcolor{lightgray!40} 1.7 &\cellcolor{lightgray!40} 2.1 &\cellcolor{lightgray!40} 1.9 &\cellcolor{lightgray!40} 1.4 & 0.8 & \cellcolor{black!40} 5.2 \\ 
  7 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 0.6 & 0.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.5 &\cellcolor{lightgray!40} 1.1 &\cellcolor{lightgray!40} 1.4 &\cellcolor{lightgray!40} 1.3 & 0.9 & 0.6 &\cellcolor{lightgray!40} 3.8 \\ 
  8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.2 & 0.2 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.3 & 0.6 & 0.8 & 0.8 & 0.6 & 0.3 &\cellcolor{lightgray!40} 2.4 \\ 
  9 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.3 & 0.4 & 0.4 & 0.3 & 0.2 &\cellcolor{lightgray!40} 1.3 \\ 
  10 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.1 & 0.2 & 0.2 & 0.1 & 0.1 & 0.7 \\ 
  

==> vdhmm_model_choice.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Wed May 23 09:20:59 2018
Na{\"i}ve HMM & 92076.24 & 92076.32 & 91789.71 & 40986.40 \\  
HMMX & 91725.22 & 91701.80 & 90728.74 & 40828.86 \\[0.3em] 
Na{\"i}ve VDC-HMM & 89812.19 & 89815.10 & 89546.86 & 40082.27   \\
VDC-HMMX & 89402.53 & 89400.83 & 88669.65 & \bm{39966.27} \\[0.3em] 
Patient-individual VDC-HMM ($\delta$) & 88492.01 & 88226.29 & 86277.07 & 40219.75 \\
Patient-individual VDC-HMM ($\omega$) & 88170.18 & 87863.12 & 85497.23 & 40596.50 \\

  
